Matrix Approach to Helicity States of Dirac Free Particles

We derive the free wave solutions of the Dirac equation from the viewpoint of matrix algebra. The concept of spin and the corresponding helicity states are analyzed in detail. This consideration may help the readers to study mathematical methods of relativistic quantum mechanics.

==> TSWLatexianTemp_000075.tex <==
In the previous sections, de facto, we have used an important property that
the Hamiltonian of a Dirac's free particle (\ref{d2}) commutes with the
linear momentum operator,%
\begin{equation}
\left[ \widehat{H},\ \boldsymbol{\widehat{\boldsymbol{p}}}\right] =0,
\label{s0}
\end{equation}%
in order to define the states with definite values of energy and linear
momentum. But electron has also the spin, or own internal angular momentum
\cite{Mehra1969}. The corresponding integral of motion, related to the
so-called helicity operator, will be discussed here.

\subsection{Helicity Operator}

Introducing standard $4\times 4$ spin matrices and the relativistic spin
operator \cite{Merz}, \cite{Moskalev}, \cite{Schiff}:%
\begin{equation}
\mathbf{\Sigma }=\left(
\begin{array}{cc}
\boldsymbol{\sigma } & \mathbf{0} \\
\mathbf{0} & \boldsymbol{\sigma }%
\end{array}%
\right) ,\qquad \widehat{\boldsymbol{S}}=\frac{1}{2}\boldsymbol{\Sigma },
\label{s1}
\end{equation}%
one can show that%
\begin{equation}
\left[ \widehat{H},\ \boldsymbol{\Sigma }\right] =2 \iun c\left( \boldsymbol{%
\alpha \times \widehat{\boldsymbol{p}}}\right) \neq 0. \label{s2}
\end{equation}%
Indeed, by (\ref{d2}), in components,%
\begin{eqnarray}
\left[ \widehat{H},\ \Sigma _{q}\right] &=&\left[ c\alpha _{r}\ \widehat{%
p_{r}}+mc^{2}\beta ,\ \Sigma _{q}\right] \label{s2ab} \\
&=&c\widehat{p}_{r}\left[ \alpha _{r},\ \Sigma _{q}\right] +mc^{2}\left[
\beta ,\ \Sigma _{q}\right] , \notag
\end{eqnarray}%
where%
\begin{equation}
\left[ \alpha _{r},\ \Sigma _{q}\right] =2 \iun e_{rqs}\alpha _{s},\qquad \left[
\beta ,\ \Sigma _{q}\right] =0, \label{2ba}
\end{equation}%
by the block matrix multiplication (\ref{A1}) and familiar properties of
Pauli's matrices:%
\begin{equation}
\left[ \sigma _{q},\ \sigma _{r}\right] =2 \iun e_{qrs}\sigma _{s}\qquad \left(
q,r,s=1,2,3\right) . \label{s2aba}
\end{equation}%
Here, $e_{qrs}$ is the Levi-Civita symbol \cite{LaLif3}, \cite%
{Varshalovich1988}.

As a result, we obtain
\begin{equation}
\left[ \widehat{H},\ \boldsymbol{\Sigma \cdot \widehat{\boldsymbol{p}}}%
\right] =2 \iun c\left( \boldsymbol{\alpha \times \widehat{\boldsymbol{p}}}%
\right) \boldsymbol{\cdot \widehat{\boldsymbol{p}}=0}, \label{s2a}
\end{equation}%
and the following helicity operator:%
\begin{equation}
\widehat{\Lambda }=\frac{\ \boldsymbol{\widehat{\boldsymbol{S}}\cdot
\widehat{\boldsymbol{p}}}}{\left\vert \boldsymbol{\boldsymbol{p}}\right\vert
}, \label{s4}
\end{equation}%
commutes with the Hamiltonian of Dirac's free particle: $\left[ \widehat{H}%
,\ \widehat{\Lambda }\right] =0.$ Its eigenvalues $\lambda =\pm 1/2$
correspond to the relativistic states with the projections of spin in the
directions $\pm $ $\boldsymbol{\boldsymbol{p}},$ respectively.

For a Dirac particle, only the total angular momentum operator, $\widehat{%
\boldsymbol{J}}=\widehat{\boldsymbol{L}}+\widehat{\boldsymbol{S}},$ $%
\widehat{\boldsymbol{L}}=\mathbf{r}\times \widehat{\boldsymbol{p}},$ namely,
the sum of the orbital angular momentum operator and the spin, does commute
with the Hamiltonian: $\left[ \widehat{H},\ \boldsymbol{J}\right] =0$ (see,
for example, \cite{Moskalev}, \cite{Schiff} for more details). In other
words, neither the orbital angular momentum $\widehat{\boldsymbol{L}},$ nor
spin $\widehat{\boldsymbol{S}},$ are separately integrals of motion; only
the total angular momentum $\widehat{\boldsymbol{J}}=\widehat{\boldsymbol{L}}%
+\widehat{\boldsymbol{S}}$ conserves. Therefore, the plane waves under
consideration, as states with a given energy $E$ and linear momentum $%
\boldsymbol{p},$ cannot have a definite projection of the particle spin $%
\widehat{\boldsymbol{S}}$ on an arbitrary axis, say $z=x_{3}.$ Nonetheless,
as our equations (\ref{s2a})--(\ref{s4}) show, the exceptions are the states
with projection of spin towards and opposite to the direction of the linear
momentum because $\widehat{\boldsymbol{L}}\cdot \widehat{\boldsymbol{p}}%
=\left( \mathbf{r}\times \widehat{\boldsymbol{p}}\right) \cdot \widehat{%
\boldsymbol{p}}=0$ and, therefore, $\widehat{\boldsymbol{J}}\cdot \widehat{%
\boldsymbol{p}}=\widehat{\boldsymbol{S}}\cdot \widehat{\boldsymbol{p}}.$ In
this section, we will construct these Lorentz invariant (covariant) spin
states in details.

\subsection{Nonrelativistic Helicity States}

To get started, one may recall that for the nonrelativistic spin operator
\cite{LaLif3}, \cite{Varshalovich1988}:%
\begin{equation}
\boldsymbol{\widehat{\boldsymbol{s}}}=\frac{1}{2}\boldsymbol{\sigma },
\label{s5}
\end{equation}%
say, in the frame of reference, that is moving together with the particle,
with the spin pointed out in the direction of a unit polarization vector $%
\boldsymbol{\boldsymbol{n}}=\boldsymbol{\boldsymbol{n}}\left( \theta
,\varphi \right) :$%

%\vfill
%\eject
%\newpage

\begin{eqnarray}
n_{1} &=&\sin \theta \cos \varphi , \notag \\
n_{2} &=&\sin \theta \sin \varphi , \label{s6} \\
n_{3} &=&\cos \varphi , \notag
\end{eqnarray}%
the corresponding spinors satisfy the following eigenvalue problem (helicity
states \cite{Moskalev}, \cite{Varshalovich1988}):%
\begin{equation}
\left( \widehat{\boldsymbol{s}}\boldsymbol{\cdot \boldsymbol{n}}\right) \phi
=\frac{1}{2}\left( \boldsymbol{\boldsymbol{\sigma }\cdot \boldsymbol{n}}%
\right) \phi =\lambda \phi . \label{s7}
\end{equation}%
The standard solutions are%
\begin{equation}
\phi ^{\left( 1/2\right) }\left( \theta ,\varphi \right) =\left(
\begin{array}{c}
\cos \dfrac{\theta }{2}\ e^{- \iun \varphi /2} \\
\sin \dfrac{\theta }{2}\ e^{ \iun \varphi /2}%
\end{array}%
\right) \quad \left( \text{when }\lambda =+\frac{1}{2}\right) ,\qquad \phi
^{\left( 1/2\right) }\left( 0,0\right) =\left(
\begin{array}{c}
1 \\
0%
\end{array}%
\right) ; \label{s8a}
\end{equation}%
and%
\begin{equation}
\phi ^{\left( -1/2\right) }\left( \theta ,\varphi \right) =\left(
\begin{array}{c}
-\sin \dfrac{\theta }{2}\ e^{- \iun \varphi /2} \\
\cos \dfrac{\theta }{2}\ e^{ \iun \varphi /2}%
\end{array}%
\right) \quad \left( \text{when }\lambda =-\frac{1}{2}\right) ,\qquad \phi
^{\left( 1/2\right) }\left( 0,0\right) =\left(
\begin{array}{c}
0 \\
1%
\end{array}%
\right) \label{s8b}
\end{equation}%
with the projection of spin in the direction $\pm \boldsymbol{\boldsymbol{n}}%
\left( \theta ,\varphi \right) ,$ respectively.

As a result, in compact form,%
\begin{equation}
\left( \boldsymbol{\boldsymbol{\sigma }\cdot \boldsymbol{n}}\right) \phi
^{\left( \pm 1/2\right) }=\pm \phi ^{\left( \pm 1/2\right) }, \label{s8bb}
\end{equation}%
and, vice versa,%
\begin{equation}
\left( \phi ^{\left( \pm 1/2\right) }\right) ^{\dag }\left( \boldsymbol{%
\boldsymbol{\sigma }}\phi ^{\left( \pm 1/2\right) }\right) =\pm \boldsymbol{%
\boldsymbol{n}}=\pm \boldsymbol{\boldsymbol{n}}\left( \theta ,\varphi
\right) . \label{s8bc}
\end{equation}%
These facts can be verified by direct substitutions (details are left to the
reader).

Both nonrelativistic helicity states can be thought of as the columns of the
following $2\times 2$ unitary matrix;%
\begin{equation}
\Phi =\left( \phi ^{\left( 1/2\right) },\ \phi ^{\left( -1/2\right) }\right)
=\left(
\begin{array}{cc}
\cos \dfrac{\theta }{2}e^{- \iun \varphi /2} & -\sin \dfrac{\theta }{2}%
e^{- \iun \varphi /2} \\
\sin \dfrac{\theta }{2}e^{ \iun \varphi /2} & \cos \dfrac{\theta
	}{2}e^{ \iun \varphi
/2}%
\end{array}%
\right) ,\qquad \Phi \ \Phi ^{\dag }=\boldsymbol{1}, \label{s8c}
\end{equation}%
which is related to the spin $1/2$ finite rotation matrix \cite{LaLif3},
\cite{Varshalovich1988}. Introducing also,%
\begin{equation}
\widetilde{\Phi }=\left( \phi ^{\left( 1/2\right) },\ -\phi ^{\left(
-1/2\right) }\right) =\left(
\begin{array}{cc}
\cos \dfrac{\theta }{2}e^{- \iun \varphi /2} & \sin \dfrac{\theta }{2}%
e^{- \iun \varphi /2} \\
\sin \dfrac{\theta }{2}e^{ \iun \varphi /2} & -\cos \dfrac{\theta
	}{2}e^{ \iun \varphi
/2}%
\end{array}%
\right) ,\qquad \widetilde{\Phi }\ \widetilde{\Phi }^{\dag }=\boldsymbol{1},
\label{s8d}
\end{equation}%
we will establish the following factorization properties of the helicity
matrix:%
\begin{equation}
\boldsymbol{\boldsymbol{\sigma }\cdot \boldsymbol{n}}=\widetilde{\Phi }\
\Phi ^{\dag }=\Phi \ \widetilde{\Phi }\ ^{\dag }. \label{s8e}
\end{equation}%
Indeed, rewriting in the right-hand side, say $\widetilde{\Phi }\ \Phi
^{\dag },$ in explicit form, one gets:%
\begin{eqnarray}
&&\left(
\begin{array}{cc}
\cos \dfrac{\theta }{2}e^{- \iun \varphi /2} & \sin \dfrac{\theta }{2}%
e^{- \iun \varphi /2} \\
\sin \dfrac{\theta }{2}e^{ \iun \varphi /2} & -\cos \dfrac{\theta
	}{2}e^{ \iun \varphi
/2}%
\end{array}%
\right) \left(
\begin{array}{cc}
\cos \dfrac{\theta }{2}e^{ \iun \varphi /2} & \sin \dfrac{\theta
	}{2}e^{- \iun \varphi
/2} \\
-\sin \dfrac{\theta }{2}e^{ \iun \varphi /2} & \cos \dfrac{\theta }{2}%
e^{- \iun \varphi /2}%
\end{array}%
\right) \label{s8f} \\
&&\qquad \qquad \qquad \qquad \qquad =\left(
\begin{array}{cc}
\cos \theta & \sin \theta \ e^{- \iun \varphi } \\
\sin \theta \ e^{ \iun \varphi } & -\cos \theta%
\end{array}%
\right) =\boldsymbol{\boldsymbol{\sigma }\cdot \boldsymbol{n}}, \notag
\end{eqnarray}%
by the familiar double-angle trigonometric identities. As a result, the
eigenvalue problem (\ref{s7}), or (\ref{s8bb}), is verified:%
\begin{equation}
\left( \boldsymbol{\boldsymbol{\sigma }\cdot \boldsymbol{n}}\right) \Phi
=\left( \widetilde{\Phi }\ \Phi ^{\dag }\right) \Phi =\widetilde{\Phi }%
\left( \Phi ^{\dag }\Phi \right) =\widetilde{\Phi }, \label{s8g}
\end{equation}%
by a simple matrix multiplication. Thus,%
\begin{equation}
\left( \boldsymbol{\boldsymbol{\sigma }\cdot \boldsymbol{n}}\right) \Phi =%
\widetilde{\Phi },\qquad \left( \boldsymbol{\boldsymbol{\sigma }\cdot
\boldsymbol{n}}\right) \widetilde{\Phi }=\Phi , \label{s8h}
\end{equation}%
say, due to a familiar relation $\left( \boldsymbol{\sigma \cdot n}\right)
^{2}=\mathbf{1}.$ (We haven't been able to find these calculations in the
available literature.)
%
%

\textbf{Note}. Introducing the spin one-half polarization density matrix as
follows%
\begin{equation}
\rho _{rs}^{\left( \lambda \right) }\left( \boldsymbol{\boldsymbol{n}}%
\right) :=\phi _{r}^{\left( \lambda \right) }\left( \boldsymbol{\boldsymbol{n%
}}\right) \left[ \phi _{s}^{\left( \lambda \right) }\left( \boldsymbol{%
\boldsymbol{n}}\right) \right] ^{\ast }\qquad \left( r,s=1,2\right) ,
\label{s8aa}
\end{equation}
one gets%
\begin{equation}
\rho ^{\left( \pm 1/2\right) }\left( \boldsymbol{\boldsymbol{n}}\right) =%
\frac{1}{2}\left( \mathbf{1}\pm \boldsymbol{\sigma \cdot n}\right) .
\label{s8ab}
\end{equation}%
(More details can be found in \cite{LaLif3}, \cite{Moskalev}, \cite%
{Varshalovich1988}.) \ \ \ $\blacksquare $

\subsection{Relativistic Plane Waves}

Let us extend the original solutions (\ref{ma6}) and analyze them from a
different perspective. For a free relativistic particle with the linear
momentum $\boldsymbol{\boldsymbol{p}}$ and energy $E,$ one can look for
solutions of (\ref{d9}) in the block form%
\begin{equation}
v\left( p\right) =C\left(
\begin{array}{c}
\phi \\
\chi%
\end{array}%
\right) , \label{s9}
\end{equation}%
where $C$ is a constant and $\phi ,$ $\chi $ are two-component spinors:%
\begin{equation}
\phi =\left(
\begin{array}{c}
\phi _{1} \\
\phi _{2}%
\end{array}%
\right) ,\qquad \chi =\left(
\begin{array}{c}
\chi _{1} \\
\chi _{2}%
\end{array}%
\right) . \label{s10}
\end{equation}%
Then%
\begin{eqnarray}
\left( mc^{2}-E\right) \phi +c\left( \boldsymbol{\sigma \cdot p}\right) \chi
&=&0, \label{s11} \\
c\left( \boldsymbol{\sigma \cdot p}\right) \phi -\left( mc^{2}+E\right) \chi
&=&0. \notag
\end{eqnarray}%
From the second (first) equation:%
\begin{equation}
\chi =\frac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi
\qquad \left( \phi =\frac{c\left( \boldsymbol{\sigma \cdot p}\right) }{%
E-mc^{2}}\chi \right) \label{s12}
\end{equation}%
and the substitution of this relation into the first (second) equation gives
the relativistic spectrum (\ref{ma4}) for a spinor $\phi $ (correspondingly,
$\chi $) related to an arbitrary polarization vector $\boldsymbol{%
\boldsymbol{n}},$ in the frame of reference where the particle is at rest.
[Substitution of the second relation (\ref{s12}) into the first one results
in an identity on the spectrum (\ref{ma4}), and vise versa.]

As a result, the general solutions under consideration have the forms \cite%
{Moskalev}:%
\begin{equation}
v\left( p\right) =C\left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) \quad \qquad \left( \text{and }D\left(
\begin{array}{c}
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}-E}\chi \\
-\chi%
\end{array}%
\right) \right) . \label{s13}
\end{equation}

\textbf{Note}. These formulas can also be obtained by the (inverse) Lorentz
boost towards to the direction $\boldsymbol{\boldsymbol{l}}=\boldsymbol{%
\boldsymbol{p/}}\left\vert \boldsymbol{\boldsymbol{p}}\right\vert $ from the
frame of reference when the particle is at rest. Indeed, the system (\ref%
{s11}) has a trivial solution $E=mc^{2},$ $\boldsymbol{p}=\boldsymbol{0}$
and $\chi =0$ with an arbitrary spinor $\phi .$ The above transformation of
energy and momentum takes the form:%
\begin{equation}
\left(
\begin{array}{c}
E/c \\
\left\vert \boldsymbol{\boldsymbol{p}}\right\vert%
\end{array}%
\right) =\left(
\begin{array}{cc}
\cosh \vartheta & \sinh \vartheta \\
\sinh \vartheta & \cosh \vartheta%
\end{array}%
\right) \left(
\begin{array}{c}
mc \\
0%
\end{array}%
\right) , \label{s13aa}
\end{equation}%
or $E=mc^{2}\cosh \vartheta $ and $\left\vert \boldsymbol{\boldsymbol{p}}%
\right\vert =mc\sinh \vartheta .$ For positive energy eigenvalues, one gets
\begin{eqnarray}
v\left( p\right) &=&S_{L^{-1}}v\left( \boldsymbol{\boldsymbol{p}}=\mathbf{0}%
\right) =e^{-\vartheta \left( \boldsymbol{\sigma \cdot l}\right) /2}v\left(
0\right) =\left( \cosh \frac{\vartheta }{2}+\left( \boldsymbol{\alpha \cdot l%
}\right) \sinh \frac{\vartheta }{2}\right) v\left( 0\right) \label{s13a} \\
&=&\left(
\begin{array}{cc}
\cosh \dfrac{\vartheta }{2} & \left( \boldsymbol{\sigma \cdot l}\right)
\sinh \dfrac{\vartheta }{2} \\
\left( \boldsymbol{\sigma \cdot l}\right) \sinh \dfrac{\vartheta }{2} &
\cosh \dfrac{\vartheta }{2}%
\end{array}%
\right) \left(
\begin{array}{c}
\phi \\
0%
\end{array}%
\right) =\cosh \dfrac{\vartheta }{2}\left(
\begin{array}{c}
\phi \\
\left( \boldsymbol{\sigma \cdot l}\right) \tanh \dfrac{\vartheta }{2}\ \phi%
\end{array}%
\right) \notag
\end{eqnarray}%
(see, for example, \cite{BerLifPit}, \cite{Kr:Lan:Sus16}, \cite{Kr:Lan:Sus60}%
, \cite{Moskalev}, \cite{PeskSchroe}, \cite{Steane2012}, \cite{Steane} for
more details). Here,%
\begin{equation}
\cosh \dfrac{\vartheta }{2}=\sqrt{\frac{\cosh \vartheta +1}{2}}=\sqrt{\frac{%
E+mc^{2}}{2mc^{2}}},\qquad \tanh \dfrac{\vartheta }{2}=\frac{\sinh \vartheta
}{\cosh \vartheta +1}=\frac{c\left\vert \boldsymbol{\boldsymbol{p}}%
\right\vert }{E+mc^{2}}. \label{s13ab}
\end{equation}%
Once again, we obtain the first equation (\ref{s13}) with $C=\sqrt{\left(
mc^{2}+E\right) /2mc^{2}}.$ \ \ $\ \blacksquare $

\subsection{Relativistic Polarization Vector}

We follow \cite{AkhBer}, \cite{Moskalev} with somewhat different details. In
covariant form, the Dirac equation (\ref{d1})-(\ref{d2}) can be written as
follows%
\begin{equation}
\left( \gamma ^{\mu }\widehat{p}_{\mu }-mc\right) \psi =0,\qquad \widehat{p}%
_{\mu }= \iun \hbar \frac{\partial }{\partial x^{\mu }}, \label{rd1}
\end{equation}%
where $x^{\mu }=\left( ct,\boldsymbol{r}\right) ,$ $\gamma ^{\mu }=\left(
\gamma ^{0},\boldsymbol{\gamma }\right) ,$ and%
\begin{equation}
\gamma ^{0}=\beta =\left(
\begin{array}{cc}
\mathbf{1} & \mathbf{0} \\
\mathbf{0} & -\mathbf{1}%
\end{array}%
\right) ,\qquad \boldsymbol{\gamma }=\beta \boldsymbol{\alpha }=\left(
\begin{array}{cc}
\mathbf{0} & \mathbf{\sigma } \\
-\mathbf{\sigma } & \mathbf{0}%
\end{array}%
\right) . \label{rd2}
\end{equation}%
Throughout the article, we use Einstein's summation convention:%
\begin{equation}
a^{\mu }b_{\mu }=g_{\mu \nu }a^{\mu }b^{\nu
}=a^{0}b_{0}+a^{1}b_{1}+a^{2}b_{2}+a^{3}b_{3}=a^{0}b_{0}-\boldsymbol{a\cdot b%
}, \label{rd3}
\end{equation}%
when $a^{\mu }=\left( a^{0},\boldsymbol{a}\right) $ and $b_{\mu }=g_{\mu \nu
}b^{\nu }=\left( b^{0},-\boldsymbol{b}\right) ,$ unless stated otherwise
(see, for example, \cite{Kr:Lan:Sus16} and \cite{Moskalev} for more
details). Here, $g_{\mu \nu }=g^{\mu \nu }=$diag$(1,-1,-1,-1)$ is the
pseudo-Euclidean metric of Minkowski space and the familiar anticommutation
relation holds%
\begin{equation}
\gamma ^{\mu }\gamma ^{\nu }+\gamma ^{\nu }\gamma ^{\mu }=2g^{\mu \nu
}\qquad \left( \mu ,\nu =0,1,2,3\right) . \label{rd3a}
\end{equation}

The bi-spinor wave function for a free Dirac particle, corresponding to a
given energy-momentum four vector, $p_{\mu }=\left( E/c,-\boldsymbol{p}%
\right) $ with the relativistic invariant $p_{\mu }p^{\mu }=\left(
E/c\right) ^{2}-\boldsymbol{p}^{2}=m^{2}c^{2}$ in covariant form, is given by%
\begin{equation}
\psi \left( x\right) =u\left( p\right) e^{- \iun \left( p_{\mu }x^{\mu }\right)
/\hbar },\qquad E=+R=\sqrt{c^{2}\boldsymbol{p}^{2}+m^{2}c^{4}}>0,
\label{rd4}
\end{equation}%
and the standard normalization is as follows%
\begin{equation}
\overline{u}\left( p\right) u\left( p\right) =1,\qquad \overline{u}\left(
p\right) =u^{\dag }\left( p\right) \gamma ^{0}. \label{rd5}
\end{equation}%
The matrix equations for $u\left( p\right) $ and $\overline{u}\left(
p\right) $ take the form \cite{Moskalev}:%
\begin{equation}
\left( \gamma ^{\mu }p_{\mu }-mc\right) u\left( p\right) =0,\qquad \overline{%
u}\left( p\right) \left( \gamma ^{\mu }p_{\mu }-mc\right) =0. \label{rd5a}
\end{equation}%
The normalized bi-spinor is given by%
\begin{equation}
u\left( p\right) =\sqrt{\frac{E+mc^{2}}{2mc^{2}}}\left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) , \label{rd6}
\end{equation}%
for an arbitrary normalized spinor $\phi :$%
\begin{equation}
\phi ^{\dag }\phi =\left( \phi _{1}^{\ast },\phi _{2}^{\ast }\right) \left(
\begin{array}{c}
\phi _{1} \\
\phi _{2}%
\end{array}%
\right) =\left\vert \phi _{1}\right\vert ^{2}+\left\vert \phi
_{2}\right\vert ^{2}=1. \label{rd7}
\end{equation}%
Indeed, by definition (\ref{rd5}),%
\begin{eqnarray}
&&\left( \phi ^{\dag },\phi ^{\dag }\dfrac{c\left( \boldsymbol{\sigma \cdot p%
}\right) }{mc^{2}+E}\right) \left(
\begin{array}{cc}
\mathbf{1} & \mathbf{0} \\
\mathbf{0} & -\mathbf{1}%
\end{array}%
\right) \left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) \label{rd8} \\
&&\,=\left( \phi ^{\dag },-\phi ^{\dag }\dfrac{c\left( \boldsymbol{\sigma
\cdot p}\right) }{mc^{2}+E}\right) \left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) =\phi ^{\dag }\phi -\phi ^{\dag }\dfrac{c^{2}\left( \boldsymbol{%
\sigma \cdot p}\right) ^{2}}{\left( mc^{2}+E\right) ^{2}}\phi \notag \\
&&\,\,=\phi ^{\dag }\phi \left( 1-\dfrac{c^{2}\boldsymbol{p}^{2}}{\left(
mc^{2}+E\right) ^{2}}\right) =\frac{2mc^{2}}{E+mc^{2}}=\frac{1}{\left\vert
C\right\vert ^{2}}. \notag
\end{eqnarray}

Let the spin of the particle be in a certain direction $\boldsymbol{n},$ in
the frame when the particle is at rest, namely,%
\begin{equation}
\left( \boldsymbol{\sigma \cdot n}\right) \phi =\phi ,\qquad \phi ^{\dag }%
\boldsymbol{\sigma }\phi =\boldsymbol{n}. \label{rd9}
\end{equation}%
[The last equation gives the expectation values of nonrelativistic spin
operator (\ref{s5}) in this frame of reference.] Introducing the
relativistic polarization (pseudo) vector as follows \cite{AkhBer}, \cite%
{Moskalev}, \cite{Rose61}, \cite{Tolhoek56}:\footnote{%
Note that $\boldsymbol{\alpha }\gamma ^{5}=\mathbf{\Sigma }.$}
\begin{equation}
a^{\mu }=\overline{\psi }\left( x\right) \left( \gamma _{5}\gamma ^{\mu
}\right) \psi \left( x\right) =\overline{u}\left( p\right) \left( \gamma
_{5}\gamma ^{\mu }\right) u\left( p\right) ,\quad \gamma ^{5}=
	\iun \gamma
^{0}\gamma ^{1}\gamma ^{2}\gamma ^{3}=\left(
\begin{array}{cc}
\mathbf{0} & \mathbf{1} \\
\mathbf{1} & \mathbf{0}%
\end{array}%
\right) =-\gamma _{5}, \label{rd9rd}
\end{equation}%
one can derive the components of this polarization four vector $a^{\mu
}=\left( a^{0},\boldsymbol{a}\right) :$%
\begin{equation}
a^{0}=\frac{\left( \boldsymbol{p\cdot n}\right) }{mc},\qquad \boldsymbol{a}=%
\boldsymbol{n}+\frac{\boldsymbol{p}\left( \boldsymbol{p\cdot n}\right) }{%
m\left( E+mc^{2}\right) }. \label{rd10}
\end{equation}%
Here, the following properties of Pauli's matrices,%
\begin{equation}
\left( \boldsymbol{\sigma \cdot p}\right) \left( \boldsymbol{\sigma \cdot n}%
\right) = \iun \left( \boldsymbol{p\times n}\right) \cdot \boldsymbol{\sigma }%
+\left( \boldsymbol{p\cdot n}\right) \label{rd10a}
\end{equation}%
and%
\begin{equation}
\left( \boldsymbol{\sigma \cdot p}\right) \boldsymbol{\sigma }\left(
\boldsymbol{\sigma \cdot p}\right) =2\boldsymbol{p}\left( \boldsymbol{\sigma
\cdot p}\right) -\boldsymbol{p}^{2}\boldsymbol{\sigma }, \label{rd11}
\end{equation}%
should be utilized along with (\ref{rd9}). [These identities can be verified
with the aid of commutator relations (\ref{s2aba}).]

By definition (\ref{rd9rd}), in components,%
\begin{eqnarray}
a^{0} &=&\left\vert C\right\vert ^{2}\left( \phi ^{\dag },-\phi ^{\dag }%
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\right) \left(
\begin{array}{cc}
\mathbf{0} & \mathbf{1} \\
-\mathbf{1} & \mathbf{0}%
\end{array}%
\right) \left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) \label{rd11a} \\
&=&\left\vert C\right\vert ^{2}\left( \phi ^{\dag },-\phi ^{\dag }\dfrac{%
c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\right) \left(
\begin{array}{c}
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi \\
-\phi%
\end{array}%
\right) =\frac{2c\left\vert C\right\vert ^{2}}{E+mc^{2}}\phi ^{\dag }\left(
\boldsymbol{\sigma \cdot p}\right) \left( \boldsymbol{\sigma \cdot n}\right)
\phi \notag \\
&=&\dfrac{1}{mc}\phi ^{\dag }\left(  \iun \left( \boldsymbol{p\times n}\right)
\cdot \boldsymbol{\sigma }+\left( \boldsymbol{p\cdot n}\right) \right) \phi =%
\dfrac{1}{mc}\left( \left( \boldsymbol{p\cdot n}\right) + \iun \left( \boldsymbol{%
p\times n}\right) \cdot \boldsymbol{n}\right) =\dfrac{\boldsymbol{p\cdot n}}{%
mc}. \notag
\end{eqnarray}%
In a similar fashion,%
\begin{eqnarray}
\boldsymbol{a} &=&\left\vert C\right\vert ^{2}\left( \phi ^{\dag },-\phi
^{\dag }\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\right)
\left(
\begin{array}{cc}
\mathbf{\sigma } & \mathbf{0} \\
\mathbf{0} & -\mathbf{\sigma }%
\end{array}%
\right) \left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) \label{rd11b} \\
&=&\left\vert C\right\vert ^{2}\left( \phi ^{\dag },-\phi ^{\dag }\dfrac{%
c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\right) \left(
\begin{array}{c}
\mathbf{\sigma }\phi \\
-\mathbf{\sigma }\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E%
}\phi%
\end{array}%
\right) \notag \\
&=&\left\vert C\right\vert ^{2}\left( \phi ^{\dag }\mathbf{\sigma }\phi +%
\dfrac{c^{2}}{\left( mc^{2}+E\right) ^{2}}\phi ^{\dag }\left( \boldsymbol{%
\sigma \cdot p}\right) \boldsymbol{\sigma }\left( \boldsymbol{\sigma \cdot p}%
\right) \phi \right) , \notag
\end{eqnarray}%
where%
\begin{equation*}
\phi ^{\dag }\left( \boldsymbol{\sigma \cdot p}\right) \boldsymbol{\sigma }%
\left( \boldsymbol{\sigma \cdot p}\right) \phi =2\boldsymbol{p}\left( \phi
^{\dag }\boldsymbol{\sigma }\phi \right) \boldsymbol{\cdot p}-\boldsymbol{p}%
^{2}\phi ^{\dag }\boldsymbol{\sigma }\phi ,
\end{equation*}%
in view of identity (\ref{rd11}). As a result,%
\begin{eqnarray}
\boldsymbol{a} &=&\left\vert C\right\vert ^{2}\left( \boldsymbol{n}+\dfrac{%
c^{2}}{\left( mc^{2}+E\right) ^{2}}\left( 2\boldsymbol{p}\left( \boldsymbol{%
n\cdot p}\right) -\boldsymbol{p}^{2}\boldsymbol{n}\right) \right)
\label{rd11c} \\
&=&\left\vert C\right\vert ^{2}\left( 1-\frac{c^{2}\boldsymbol{p}^{2}}{%
\left( mc^{2}+E\right) ^{2}}\right) \boldsymbol{n}+\dfrac{2c^{2}\left\vert
C\right\vert ^{2}}{\left( mc^{2}+E\right) ^{2}}\boldsymbol{p}\left(
\boldsymbol{n\cdot p}\right) \notag \\
&=&\boldsymbol{n}+\frac{\boldsymbol{p}\left( \boldsymbol{p\cdot n}\right) }{%
m\left( E+mc^{2}\right) } \notag
\end{eqnarray}%
by (\ref{rd9}), as stated above.

The four vector (\ref{rd9rd})--(\ref{rd10}) has an important feature,
namely, in the frame of reference, when the particle is at rest, $%
\boldsymbol{p}=\boldsymbol{0},$ one gets%
\begin{equation}
a^{0}=0,\qquad \boldsymbol{a}=\boldsymbol{n}, \label{rd12}
\end{equation}%
thus extending the particle nonrelativistic $3D$ polarization (preudo)
vector. And vice versa, the polarization four vector (\ref{rd10}) can be
obtained from the latter one by the Lorentz transformation \cite{BerLifPit}.

Moreover, the four vector $a^{\mu }$ has the following properties:%
\begin{equation}
p_{\mu }a^{\mu }=0,\qquad a^{2}=a_{\mu }a^{\mu }=-\boldsymbol{n}^{2}=-1.
\label{rd12a}
\end{equation}%
Indeed, by definition (\ref{rd9rd}) and Dirac's equations for bi-spinors $%
u\left( p\right) $, $\overline{u}\left( p\right) ,$ namely (\ref{rd5a}), one
gets%
\begin{eqnarray}
p_{\mu }a^{\mu } &=&\overline{u}\left( p\right) \gamma _{5}\left( p_{\mu
}\gamma ^{\mu }\right) u\left( p\right) =\frac{1}{2}\overline{u}\left(
p\right) \left( \gamma _{5}\left( p_{\mu }\gamma ^{\mu }\right) -\left(
p_{\mu }\gamma ^{\mu }\right) \gamma _{5}\right) u\left( p\right) \notag \\
&=&\frac{1}{2}\overline{u}\left( p\right) \left( \gamma _{5}mc-mc\gamma
_{5}\right) u\left( p\right) =0 \label{rd12aa}
\end{eqnarray}%
in view of a familiar anticommutator relation $\gamma ^{\mu }\gamma
_{5}+\gamma _{5}\gamma ^{\mu }=0$ $\left( \mu =0,1,2,3\right) $. [This
covariant orthogonality relation can be directly verified with the help of (%
\ref{rd10}) and/or evaluated in the frame of reference, when the particle is
at rest, see (\ref{rd12}).]

It worth noting that the bi-spinor $u\left( p\right) ,$ corresponding to the
Dirac free particle with the relativistic polarization vector $a^{\mu },$ in
addition to the Dirac equation,%
\begin{equation}
\left( \gamma ^{\mu }p_{\mu }-mc\right) u\left( p\right) =0, \label{rd12b}
\end{equation}%
also does satisfy the following matrix equation,%
\begin{equation}
\left( \gamma _{5}\gamma ^{\mu }a_{\mu }+I\right) u\left( p\right) =0,
\label{rd12c}
\end{equation}%
which can be verified by direct substitution of $u\left( p\right) $ from (%
\ref{rd6}). [The latter can be thought of as a relativistic generalization
of the first equation (\ref{rd9}), because they coincide when $\boldsymbol{p}%
=\boldsymbol{0}.]$ Indeed, up to a given normalization,%
\begin{eqnarray}
&&\left( \gamma _{5}\gamma ^{\mu }a_{\mu }+I\right) u\left( p\right) =\left(
\begin{array}{cc}
\mathbf{1}-\boldsymbol{\sigma \cdot a} & a^{0} \\
-a^{0} & \mathbf{1}+\boldsymbol{\sigma \cdot a}%
\end{array}%
\right) C\left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) \label{rd12dd} \\
&&\,=C\left(
\begin{array}{c}
\phi -\left( \boldsymbol{\sigma \cdot a}\right) \phi +a^{0}\dfrac{c\left(
\boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi \\
-a^{0}\phi +\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}%
\phi +\dfrac{c\left( \boldsymbol{\sigma \cdot a}\right) \left( \boldsymbol{%
\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) \notag \\
&&\,=C\left(
\begin{array}{c}
\phi -\left( \boldsymbol{\sigma \cdot n}\right) \phi -\dfrac{\left(
\boldsymbol{\sigma \cdot p}\right) \left( \boldsymbol{p\cdot n}\right) }{%
m\left( mc^{2}+E\right) }\phi +\dfrac{\left( \boldsymbol{p\cdot n}\right)
\left( \boldsymbol{\sigma \cdot p}\right) }{m\left( mc^{2}+E\right) }\phi =0
\\
-\dfrac{\left( \boldsymbol{p\cdot n}\right) }{mc}\phi +c\dfrac{\left(
\boldsymbol{\sigma \cdot p}\right) \left( \boldsymbol{\sigma \cdot n}\right)
+\left( \boldsymbol{\sigma \cdot n}\right) \left( \boldsymbol{\sigma \cdot p}%
\right) }{mc^{2}+E}\phi +\dfrac{\left( \boldsymbol{p\cdot n}\right) c^{2}%
\boldsymbol{p}^{2}}{mc\left( mc^{2}+E\right) ^{2}}\phi \\
=-\dfrac{\left( \boldsymbol{p\cdot n}\right) }{mc}\phi +\dfrac{2c\left(
\boldsymbol{p\cdot n}\right) }{E+mc^{2}}\phi +\dfrac{\left( \boldsymbol{%
p\cdot n}\right) \left( E^{2}-m^{2}c^{4}\right) }{mc\left( E+mc^{2}\right)
^{2}}\phi \\
=\dfrac{\left( \boldsymbol{p\cdot n}\right) }{mc}\left( -1+\dfrac{2mc^{2}}{%
E+mc^{2}}+\dfrac{E-mc^{2}}{E+mc^{2}}\right) \phi =0%
\end{array}%
\right) \notag
\end{eqnarray}%
by (\ref{rd9}) and (\ref{rd10})--(\ref{rd10a}).

It worth mentioning, in conclusion, that the current density four vector for
a free Dirac particle with a definite energy and linear momentum is given by%
\begin{equation}
j^{\mu }=\overline{\psi }\left( x\right) \left( \gamma ^{\mu }\right) \psi
\left( x\right) =\overline{u}\left( p\right) \left( \gamma ^{\mu }\right)
u\left( p\right) =\frac{p^{\mu }}{mc}\overline{u}\left( p\right) u\left(
p\right) \label{rd12d}
\end{equation}%
for an arbitrary normalization of the spinor $\phi $ in (\ref{rd6}) (see
\cite{Moskalev} for more details).

\subsection{Expectation Values of Relativistic Spin Operator}

Let%
\begin{equation}
\ \left\langle \boldsymbol{\widehat{\boldsymbol{S}}}\right\rangle =\frac{%
u^{\dag }\left( \frac{1}{2}\mathbf{\Sigma }\right) u}{u^{\dag }u},\qquad
\left\langle \boldsymbol{\widehat{\boldsymbol{s}}}\right\rangle =\frac{\phi
^{\dag }\left( \frac{1}{2}\mathbf{\sigma }\right) \phi }{\phi ^{\dag }\phi }
\label{sr1}
\end{equation}%
be expectation values for the relativistic, when $\boldsymbol{p\neq }\mathbf{%
0},$ and nonrelativistic, if $\boldsymbol{p=}\mathbf{0},$ spin operators for
a Dirac particle, respectively, \cite{Moskalev}. Then
%
{\footnote{This result follows also from (\ref{rd9rd})--(\ref{rd10})}}
%
\begin{equation}
\ \left\langle \boldsymbol{\widehat{\boldsymbol{S}}}\right\rangle =\frac{%
mc^{2}}{E}\left\langle \boldsymbol{\widehat{\boldsymbol{s}}}\right\rangle +%
\frac{c^{2}\boldsymbol{p}}{E\left( E+mc^{2}\right) }\left( \boldsymbol{%
p\cdot }\left\langle \boldsymbol{\widehat{\boldsymbol{s}}}\right\rangle
\right) . \label{sr2}
\end{equation}%
Indeed, for bi-spinor (\ref{rd6}), up to a constant,%
\begin{eqnarray}
u^{\dag }\left( \mathbf{\Sigma }\right) u &=&\left( \phi ^{\dag },\phi
^{\dag }\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\right)
\left(
\begin{array}{cc}
\mathbf{\sigma } & \mathbf{0} \\
\mathbf{0} & \mathbf{\sigma }%
\end{array}%
\right) \left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) \label{sr3} \\
&=&\left( \phi ^{\dag },\phi ^{\dag }\dfrac{c\left( \boldsymbol{\sigma \cdot
p}\right) }{mc^{2}+E}\right) \left(
\begin{array}{c}
\mathbf{\sigma }\phi \\
\mathbf{\sigma }\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}%
\phi%
\end{array}%
\right) \notag \\
&=&\phi ^{\dag }\mathbf{\sigma }\phi +\frac{c^{2}}{\left( E+mc^{2}\right)
^{2}}\phi ^{\dag }\left[ \left( \boldsymbol{\sigma \cdot p}\right) \mathbf{%
\sigma }\left( \boldsymbol{\sigma \cdot p}\right) \right] \phi . \notag
\end{eqnarray}%
In view of (\ref{rd11}), one gets%
\begin{equation}
u^{\dag }\left( \mathbf{\Sigma }\right) u=\frac{2mc^{2}}{E+mc^{2}}\left[
\left( \phi ^{\dag }\mathbf{\sigma }\phi \right) +\frac{\boldsymbol{p}}{%
m\left( E+mc^{2}\right) }\boldsymbol{p\cdot }\left( \phi ^{\dag }\mathbf{%
\sigma }\phi \right) \right] . \label{sr4}
\end{equation}%
In a similar fashion, up to a constant,
\begin{equation}
u^{\dag }u=\frac{2E}{E+mc^{2}}\left( \phi ^{\dag }\phi \right) . \label{sr5}
\end{equation}%
As a result, we obtain (\ref{sr2}).

In a special case, when the $z$-axis is directed towars $\boldsymbol{p},$
one gets%
\begin{equation}
\ \left\langle \widehat{S_{x}}\right\rangle =\frac{mc^{2}}{E}\left\langle
\widehat{s_{x}}\right\rangle ,\qquad \ \left\langle \widehat{S_{y}}%
\right\rangle =\frac{mc^{2}}{E}\left\langle \widehat{s_{y}}\right\rangle
,\qquad \ \left\langle \widehat{S_{z}}\right\rangle =\left\langle \widehat{%
s_{z}}\right\rangle \label{sr6}
\end{equation}%
(see \cite{Moskalev} for more details).

\subsection{Relativistic Helicity States}

When the spinor $\phi $ (respectively, $\chi $) corresponds to the
nonrelativistic helicity states (\ref{s7})--(\ref{s8b}) with the particular
polarization vector $\boldsymbol{\boldsymbol{n}}=\boldsymbol{\boldsymbol{p/}}%
\left\vert \boldsymbol{\boldsymbol{p}}\right\vert $ (in the frame of
reference where the particle is at rest), the bi-spinors (\ref{s13}) become
the common eigenfunctions of the commuting Hamiltonian and helicity
operator: $\left[ \widehat{H},\ \Lambda \right] =0.$ For example, up to a
normalization,%
\begin{eqnarray}
\left( \boldsymbol{\Sigma \cdot \boldsymbol{p}}\right) v\left( p\right)
&=&C\left(
\begin{array}{cc}
\boldsymbol{\sigma \cdot p} & \boldsymbol{0} \\
\boldsymbol{0} & \boldsymbol{\sigma \cdot p}%
\end{array}%
\right) \left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) \label{s14} \\
&=&C\left(
\begin{array}{c}
\left( \boldsymbol{\sigma \cdot p}\right) \phi \\
\left( \boldsymbol{\sigma \cdot p}\right) \dfrac{c\left( \boldsymbol{\sigma
\cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) =2\lambda \left\vert \boldsymbol{\boldsymbol{p}}\right\vert C\left(
\begin{array}{c}
\phi \\
\dfrac{c\left( \boldsymbol{\sigma \cdot p}\right) }{mc^{2}+E}\phi%
\end{array}%
\right) , \notag
\end{eqnarray}%
or%
\begin{equation}
\widehat{\Lambda }v\left( p\right) =\lambda v\left( p\right) \label{s15}
\end{equation}%
for our both helicity states (\ref{s13}).

Applying the block matrix multiplication rule (\ref{A1}), one gets:
%
\begin{eqnarray}
&&\left(
\begin{array}{cc}
\left( mc^{2}+E\right) \Phi & c\left( \boldsymbol{\sigma \cdot p}\right) \Phi
\\
c\left( \boldsymbol{\sigma \cdot p}\right) \Phi & -\left( mc^{2}+E\right)
\Phi%
\end{array}%
\right) ^{\dag }\left(
\begin{array}{cc}
\left( mc^{2}+E\right) \Phi & c\left( \boldsymbol{\sigma \cdot p}\right) \Phi
\\
c\left( \boldsymbol{\sigma \cdot p}\right) \Phi & -\left( mc^{2}+E\right)
\Phi%
\end{array}%
\right) \label{s16} \\
&&\quad =\left(
\begin{array}{cc}
\left( mc^{2}+E\right) \Phi ^{\dag } & c\Phi ^{\dag }\left( \boldsymbol{%
\sigma \cdot p}\right) \\
c\Phi ^{\dag }\left( \boldsymbol{\sigma \cdot p}\right) & -\left(
mc^{2}+E\right) \Phi ^{\dag }%
\end{array}%
\right) \left(
\begin{array}{cc}
\left( mc^{2}+E\right) \Phi & c\left( \boldsymbol{\sigma \cdot p}\right) \Phi
\\
c\left( \boldsymbol{\sigma \cdot p}\right) \Phi & -\left( mc^{2}+E\right)
\Phi%
\end{array}%
\right) \notag \\
&&\qquad \qquad \qquad \qquad \qquad \qquad \qquad \qquad =\left( \left(
mc^{2}+E\right) ^{2}+c^{2}\boldsymbol{p}^{2}\right) \left(
\begin{array}{cc}
\mathbf{1} & \boldsymbol{0} \\
\boldsymbol{0} & \boldsymbol{1}%
\end{array}%
\right) \notag
\end{eqnarray}%
as an extension of our identity (\ref{ma2}). Once again, all relativistic
helicity states can be unified as the columns in the following $4\times 4$
unitary matrix:%
\begin{eqnarray}
V &=&\left( v_{+}^{\left( 1/2\right) },v_{+}^{\left( -1/2\right)
},v_{-}^{\left( 1/2\right) },v_{-}^{\left( -1/2\right) }\right) \label{s17}
\\
&=&\frac{1}{\sqrt{\left( mc^{2}+R\right) ^{2}+c^{2}\boldsymbol{p}^{2}}}%
\left(
\begin{array}{cc}
\left( mc^{2}+R\right) \Phi & c\left( \boldsymbol{\sigma \cdot p}\right) \Phi
\\
c\left( \boldsymbol{\sigma \cdot p}\right) \Phi & -\left( mc^{2}+R\right)
\Phi%
\end{array}%
\right) \notag \\
&=&\sqrt{\frac{mc^{2}+R}{2R}}\left(
\begin{array}{cc}
\Phi & \dfrac{c\left\vert \boldsymbol{\boldsymbol{p}}\right\vert }{mc^{2}+R}%
\widetilde{\Phi } \\
\dfrac{c\left\vert \boldsymbol{\boldsymbol{p}}\right\vert }{mc^{2}+R}%
\widetilde{\Phi } & -\Phi%
\end{array}%
\right) ,\qquad V^{-1}= \gamma^0 V^{\dag } \gamma^0 \notag
\end{eqnarray}%
with the help of (\ref{s8h}), that is similar to (\ref{ma6}):%
\begin{eqnarray}
V &=&\left( v_{+}^{\left( 1/2\right) },v_{+}^{\left( -1/2\right)
},v_{-}^{\left( 1/2\right) },v_{-}^{\left( -1/2\right) }\right) \label{s18}
\\
&=&\sqrt{\frac{mc^{2}+R}{2R}}\left(
\begin{array}{cc}
\left( \phi ^{\left( 1/2\right) },\ \phi ^{\left( -1/2\right) }\right) &
\dfrac{c\left\vert \boldsymbol{\boldsymbol{p}}\right\vert }{mc^{2}+R}\left(
\phi ^{\left( 1/2\right) },\ -\phi ^{\left( -1/2\right) }\right) \\
\dfrac{c\left\vert \boldsymbol{p}\right\vert }{mc^{2}+R}\left( \phi ^{\left(
1/2\right) },\ -\phi ^{\left( -1/2\right) }\right) & -\left( \phi ^{\left(
1/2\right) },\ \phi ^{\left( -1/2\right) }\right)%
\end{array}%
\right) . \notag
\end{eqnarray}%
Here, the first two columns correspond to the positive energy eigenvalues $%
E=+R=\sqrt{c^{2}\boldsymbol{p}^{2}+m^{2}c^{4}}$ and the helicities $\lambda
=\pm 1/2,$ respec\-tively. Whereas, the last two columns correspond to the
negative energy eigenvalues, given by $E=-R=-\sqrt{c^{2}\boldsymbol{p}%
^{2}+m^{2}c^{4}},$ and the helicities $\lambda =\pm 1/2,$ respec\-tively.
One should verify these facts by direct substitutions, similar to (\ref{ma7a}%
)--(\ref{ma7b}).

For the Hamiltonian $4\times 4$ matrix:%
\begin{equation}
H=c\boldsymbol{\alpha \cdot \boldsymbol{p}}+mc^{2}\beta , \label{s19}
\end{equation}%
one gets%
\begin{equation}
H^{2}=\left( c\boldsymbol{\alpha \cdot \boldsymbol{p}}+mc^{2}\beta \right)
^{2}=R^{2}=c^{2}\boldsymbol{p}^{2}+m^{2}c^{4} \label{s20}
\end{equation}%
due to the familiar anticommutators:%
\begin{equation}
\alpha _{r}\alpha _{s}+\alpha _{s}\alpha _{r}=2\delta _{rs},\qquad \alpha
_{r}\beta +\beta \alpha _{r}=0\qquad \left( r,s=1,2,3\right) . \label{s21}
\end{equation}%
As a result, we arrive at the following matrix version of the eigenvalue
problem under consideration:%
\begin{equation}
HV=R\widetilde{V},\qquad H\widetilde{V}=RV, \label{s22}
\end{equation}%
where, by definition,%
\begin{equation}
\widetilde{V}=\left( v_{+}^{\left( 1/2\right) },v_{+}^{\left( -1/2\right)
},-v_{-}^{\left( 1/2\right) },-v_{-}^{\left( -1/2\right) }\right), \qquad  {\widetilde{V}}^{-1}={\gamma}^0 {\widetilde{V}}^{\dag} {\gamma}^0 .
\label{s23}
\end{equation}%
One can obtain the following decompositions%
\begin{equation}
H=R\widetilde{V}\ V^{-1}=RV\ \widetilde{V}^{-1 } \label{s24}
\end{equation}%
similar to our factorization (\ref{s8e}) of the nonrelativistic helicity
matrix. (These results are verified in the Mathematica file.)

\subsection{Convenient Parametrization}

Following \cite{Flugge}, with somewhat different details, let us also
discuss the Dirac plane waves of positive and negative helicities $\lambda
=\pm 1/2,$ but of positive energy only, in a slightly different notation.
With%
\begin{equation}
\psi =ve^{ \iun \left( \boldsymbol{k\cdot r}-\omega t\right) } \label{h1}
\end{equation}%
and using the abbreviations%
\begin{equation}
k\eta =\frac{\omega }{c}-\frac{mc}{\hbar },\qquad \frac{k}{\eta }=\frac{%
\omega }{c}+\frac{mc}{\hbar } \label{h2}
\end{equation}%
one can express the magnitude of particle linear momentum and its kinetic
energy in terms of a suitable parameter $\eta :$%
\begin{equation}
\left\vert \boldsymbol{\boldsymbol{p}}\right\vert =\hbar k=mc\frac{2\eta }{%
1-\eta ^{2}},\qquad E=\hbar \omega =mc^{2}\frac{1+\eta ^{2}}{1-\eta ^{2}}.
\label{h3}
\end{equation}%
Once again, we use two polar angles $\theta $ and $\varphi $ in the
direction of vector $\boldsymbol{k}=\boldsymbol{p}/\hbar :$%
\begin{equation}
k_{1}\pm  \iun k_{2}=k\sin \theta \ e^{\pm  \iun \varphi },\qquad k_{3}=k\cos \theta .
\label{h4}
\end{equation}%
The eigenfunctions of the helicity operator are given by (\ref{s8a})--(\ref%
{s8b}) and (\ref{s18}) \cite{Flugge}:%
\begin{equation}
v_{+}^{\left( 1/2\right) }=\frac{1}{\sqrt{V\left( 1+\eta ^{2}\right) }}%
\left(
\begin{array}{c}
\cos \dfrac{\theta }{2}\exp \left( - \iun \dfrac{\varphi }{2}\right) \\
\sin \dfrac{\theta }{2}\exp \left(  \iun \dfrac{\varphi }{2}\right) \\
\eta \cos \dfrac{\theta }{2}\exp \left( - \iun \dfrac{\varphi }{2}\right) \\
\eta \sin \dfrac{\theta }{2}\exp \left(  \iun \dfrac{\varphi }{2}\right)%
\end{array}%
\right) \label{h5}
\end{equation}%
for $\lambda =+1/2$ and%
\begin{equation}
v_{+}^{\left( -1/2\right) }=\frac{1}{\sqrt{V\left( 1+\eta ^{2}\right) }}%
\left(
\begin{array}{c}
\sin \dfrac{\theta }{2}\exp \left( - \iun \dfrac{\varphi }{2}\right) \\
-\cos \dfrac{\theta }{2}\exp \left(  \iun \dfrac{\varphi }{2}\right) \\
-\eta \sin \dfrac{\theta }{2}\exp \left( - \iun \dfrac{\varphi }{2}\right) \\
\eta \cos \dfrac{\theta }{2}\exp \left(  \iun \dfrac{\varphi }{2}\right)%
\end{array}%
\right) \label{h6}
\end{equation}%
for $\lambda =-1/2.$ [One should compare these bi-spinors with the first two
columns in our $4\times 4$ helicity states matrix (\ref{s18}), where, in
turn, the last two columns correspond to the negative energy eigenvalues.]
Here, we use the standard normalization%
\begin{equation}
\int_{V}\overline{\psi }\gamma ^{0}\psi \ dv=\int_{V}\psi ^{\dag }\psi \
dv=\int_{V}u^{\dag }u\ dv=1. \label{h7}
\end{equation}%
It should be noted that this normalization is Lorentz-invariant, the
integral being proportional to the total electric charge inside the volume $%
V.$ (See \cite{Flugge} and \cite{Moskalev} for more details.)

In the nonrelativistic limit, when $\eta \ll 1,$ the last two components in
the above bi-spinors may be neglected and we arrive at the two-component
Pauli spin theory. The case of negative energy eigenvalues will be discussed later.
%

